DPHMs: Diffusion Parametric Head Models for Depth-based Tracking

We introduce Diffusion Parametric Head Models (DPHMs), a generative model that enables robust volumetric head reconstruction and tracking from monocular depth sequences. While recent volumetric head models, such as NPHMs, can now excel in representing high-fidelity head geometries, tracking and reconstructing heads from real-world single-view depth sequences remains very challenging, as the fitting to partial and noisy observations is underconstrained. To tackle these challenges, we propose a latent diffusion-based prior to regularize volumetric head reconstruction and tracking. This prior-based regularizer effectively constrains the identity and expression codes to lie on the underlying latent manifold which represents plausible head shapes. To evaluate the effectiveness of the diffusion-based prior, we collect a dataset of monocular Kinect sequences consisting of various complex facial expression motions and rapid transitions. We compare our method to state-of-the-art tracking methods and demonstrate improved head identity reconstruction as well as robust expression tracking.

==> latex/method_forward.tex <==

\section{Approach}
\label{SecApp}

\begin{figure*}
    \centering
    %\includegraphics[width=0.9\linewidth]{fig/latent_diffusion.png}
    \caption{\textbf{} }
  \label{fig:ldm}
\end{figure*}

\subsection{Neural Head Parametric Models}

\subsection{Latent Diffusion of Neural Head Parametric Models}

\section{Head Tracking and Reconstruction with Diffusion Priors}

\subsection{Problem Statement}

\subsection{SDS loss}

 %    \paragraph{Observation-Guided Sampling}
 % To find latent codes that can not only reconstruct the observed surface but also have faithful geometries, we have two choices:
 % (1) we can perform observation-guided latent reverse sampling. Following the reconstruction-guided sampling method in video diffusion models, we can compute the approximated observation gradient $\vec{g}$ w.r.t. a noisy code $\vec{x_t}$, defined as:
 % \begin{equation}
 %     g \leftarrow \grad_{\vec{x_t}} \lambda_{surf} \sum_j \frac{1}{2} \large( \frac{\alpha_t}{\sigma_t} \large)^{2\omega} \|F(D^{-1}(\vec{S}_j))\|^2
 % \end{equation}
 % where $\frac{\alpha_t}{\sigma_t} \large)^{2\omega}$ is a weighting factor based on signal-to-noise ratio (SNR), with a hyperparameter $\omega$. $\vec{S}$ is the observed surface. $D$ is the forward deformation decoder, and $D^{-1}$ is the iterative root finding used to find the corresponding points in the canonical space. $\|F(D^{-1}(\vec{S}_j))\|^2$ is applied to constrain the observed surface points should be on the iso-surface of canonical shape. 
 % The guidance gradients are then combined with unconditional denoising processing, expressed as a correction to the denoising output $\vec{x_t}$:
 % \begin{equation}
 %     \vec{x_t}' \leftarrow \vec{x_t} - \lambda_{gd} \frac{{\sigma_t}^2}{\alpha_t} g
 % \end{equation}

\paragraph{Diffusion Prior-constrained Optimization}
 To find latent codes that can not only reconstruct the observed surface but also have faithful geometries, we can utilize the unconditional priors to constrain the test-time optimization process of identity and expression latents.
 \begin{equation}
        L = \lambda_{surf} * L_{surf} + \lambda_{diff} * L_{diff}
  \end{equation}
$L_{diff}$ is a simplified L2 denoising loss function:
   \begin{equation}
    L_{diff} = \mathbb{E}_{t,\epsilon} \large[ \frac{1}{2}\omega_t \| \epsilon_\phi(\alpha_t\vec{x} + \sigma_t\epsilon; t) - \epsilon \|^2 \large]
\end{equation}
The gradient of $L_{diff}$:
\begin{equation}
    \grad_\vec{x} L_{diff}(\phi) = \mathbb{E}_{t, \epsilon} \left[  \omega_t (\epsilon_\phi(\vec{x_t}; t) - \epsilon) \frac{\partial\epsilon_\phi(\vec{x_t}; t)}{\vec{x_t}}  \right]
\end{equation}
Similar to dreamfusion, we can omit the Jacobian term of the denoising network (e.g. U-Net). It leads to an effective gradient for optimizing latent code $\vec{x_t}$ with diffusion models.
\begin{equation}
    \grad_\vec{x} L_{diff}(\phi) = \mathbb{E}_{t, \epsilon} \left[  \omega_t (\epsilon_\phi(\vec{x_t}; t) - \epsilon)   \right]
\end{equation}

\subsection{Identity fitting from Sparse Frames}
we use iterative root finding to warp the points from deformed expression space to the canonical space with neutral pose.

\begin{equation}
     L_{sdf} = \sum_{i=0}^{i=M}  | F(D^{-1}(\mathbf{P_{i}}, \mathbf{l^{s}}, \mathbf{l^e_{i}}), \mathbf{l^s}) |
\end{equation}

\begin{equation}
     L_{lms} = \sum_{i=0}^{i=M}  \| D(A(l^s), \mathbf{l^s}, \mathbf{l^e_{i}}) - \mathbf{L_i} \|_2^2
\end{equation}

\begin{equation}
     L_{nc} = \sum_{i=0}^{i=M}  \grad S ( {D^{-1}(\mathbf{P_i}, \mathbf{l^{s}}, \mathbf{l^e_{i}})} ) \cdot \mathbf{N_i} 
\end{equation}

\begin{equation}
\begin{aligned}
     \argmin_{\mathbf{l^{s}, \mathbf{l^e_0}, ..., \mathbf{l^e_M}}} = \lambda_{sdf} L_{sdf} + \lambda_{nc} L_{nc} + \lambda_{lms} L_{lms} + \\ \lambda_{sds} ( L_{diff}(\mathbf{l^s}) + \sum_{i=0}^{i=M}  L_{diff}(\mathbf{l^e_i}) )
\end{aligned}
\end{equation}

\subsection{Expression tracking from RGBD sequences}

\begin{equation}
     L_{p2p} = \sum_{i=0}^{i=M} \sum_{i=0}^{j=N} \min_{ k \in |\mathbf{V^s}|} \|D(\mathbf{V^s_k}, \mathbf{l^{s}}, \mathbf{l^e_{i}}) - (c * \mathbf{R_i}\mathbf{P_{ij}} + \mathbf{T_i} )\|_2^2
\end{equation}

\begin{equation}
     L_{p2l} = \sum_{i=0}^{i=M} \sum_{i=0}^{j=N} \left( D(\mathbf{V^s_k}, \mathbf{l^{s}}, \mathbf{l^e_{i}}) - (c * \mathbf{R_i}\mathbf{P_{ij}} + \mathbf{T_i} ) \right)  \cdot   (\mathbf{R_i}\mathbf{N_{ij}})
\end{equation}
%\grad S ( \mathbf{V^s_k}, \mathbf{l^s} )

\begin{equation}
     L^e_{temp} = \sum_{i=0}^{i=M-1} \| \mathbf{l^e_i}  -\mathbf{l^e_{i+1}} \|_2^2
\end{equation}

\begin{equation}
     L^{r}_{temp} = \sum_{i=0}^{i=M-1} \| \mathbf{R_i}  -\mathbf{R_{i+1}} \|_2^2 + \| \mathbf{T_i}  -\mathbf{T_{i+1}} \|_2^2
\end{equation}

\begin{equation}
\begin{aligned}
\argmin_{c, { \{ \mathbf{l^e_i}, \mathbf{R_i}, \mathbf{T_i} \} }_{i=0}^{M}} \lambda_{p2p} L_{p2p} + \lambda_{p2l} L_{p2l} +  \lambda_{nc} L_{nc} + \\\lambda_{lms} L_{lms} + \lambda^e_{temp} L^e_{temp} 
+  \lambda^r_{temp} L^r_{temp} +  \\
\lambda_{sds} ( L_{diff}(\mathbf{l^s}) + \sum_{i=0}^{i=M}  L_{diff}(\mathbf{l^e_i}) )
\end{aligned}
\end{equation}

==> rebuttal/compare_error.tex <==
\begin{figure}[!htp]
    \vspace{-0.2cm}
    \centering
    \includegraphics[width=.90\linewidth]{rebuttal/compare_temp.pdf}
    \vspace{-3mm}
    \begin{tabular}{p{5pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}}
                & (a) 
                & (b) 
                & (c) 
               & (a) 
                & (b) 
                & (c) 
    \end{tabular}
    \vspace{-3mm}
    \caption{(a) Input Scan; (b)NICP; (c)Ours. }
    \label{fig:compare_nicp}
\vspace{-5mm}
\end{figure}

\begin{figure}[!htp]
\vspace{-3mm}
    \centering
    \includegraphics[width=.8\linewidth]{rebuttal/compare_error.pdf}
    \vspace{-3mm}
    \begin{tabular}{p{5pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}}
                & 
                & NPHM
                & 
               & 
                & Ours
                & 
    \end{tabular}
    \vspace{-4mm}
    \caption{Scan2Mesh error map and result comparisons. }
    \label{fig:compare_error}
\vspace{-5mm}
\end{figure}




==> rebuttal/oneview.tex <==
\begin{wraptable}{l}{0.48\linewidth}
%\begin{table}[!htbp]
    \vspace{-4mm}
	%\renewcommand\arraystretch{1.2}
    \setlength{\tabcolsep}{1.3pt}
	\begin{center}
        \footnotesize
        %\resizebox{0.6\linewidth}{!}
        {
		\begin{tabular}{*{10}{c}}
                \toprule
			Method & FLAME   & ImFace*   & NPHM  & Ours\\ 
                \midrule
                $\ell_2$     & 2.947   & 3.065     &  1.024 & \bf 0.894\\
                NC           & 69.50     & 84.36      &  88.07 & \bf 89.02\\
                PR           & 24.21    & 31.86     &  85.88 & \bf 91.02\\
                PR2          & 55.15    & 63.29     &  97.10 & \bf 97.99\\
                %\midrule
                \bottomrule
        \end{tabular}
        }
       %\vspace{-2mm}
        % \caption{Head tracking reconstructed from single-view depths. The results are evaluated on multi-view depths. } 
        \label{tab:oneview}
        \end{center}
    \vspace{-9mm}
%\end{table}
\end{wraptable}

%scan2mesh statistics : dist_error_mean_all, 00nan norm_cosin_mean_all, 00nan fscore_mean_all, 0.265897 fscore2_mean_all, 0.551466 success subj 19, error subj 0
% error subj : []
% scan2mesh of flame statistics : dist_error_mean_all, 0.002947 norm_cosin_mean_all, 0.694973 fscore_mean_all, 0.242049 fscore2_mean_all, 0.630014 success subj 19, error subj 0
% error subj : []

% NPHM: scan2mesh statistics : dist_error_mean_all, 0.001024 norm_cosin_mean_all, 0.880740 fscore_mean_all, 0.858847 fscore2_mean_all, 0.971032 success subj 19, error subj 0

%DPHM scan2mesh statistics : dist_error_mean_all, 0.000894 norm_cosin_mean_all, 0.890199 fscore_mean_all, 0.910197 fscore2_mean_all, 0.979938 success subj 19, error subj 0




==> table/robust.tex <==
\begin{table}[!htbp]
	\renewcommand\arraystretch{1.2}
        %\setlength{\tabcolsep}{1.5pt}
        \setlength{\tabcolsep}{2pt}
	\begin{center}
        \footnotesize
		\begin{tabular}{*{9}{c}}
                \toprule
		%	 & 0 & 0.5 mm &  1mm  &  2mm\\
            \multirow{2}*{Method} & \multicolumn{2}{c}{0}   & \multicolumn{2}{c}{0.5 mm}  & \multicolumn{2}{c}{1mm} & \multicolumn{2}{c}{2mm} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  & NPHM & Ours   & NPHM & Ours   & NPHM & Ours   & NPHM & Ours 	\\
			\midrule
                \midrule
                $\ell_2$ $\downarrow$   & 1.188  & \bf 1.104 
                                        & 1.231 & \bf 1.146   
                                        & 1.271 & \bf  1.209 
                                        & 1.574 & \bf 1.392 \\
                NC $\uparrow$           & 87.56 & \bf  88.66   
                                        & 87.64 & \bf  88.58 
                                        & 86.89 & \bf  88.50  
                                        & 84.69 & \bf  88.10 \\
                RC $\uparrow$           & 84.49 &  \bf 89.87 
                                        & 82.93 &  \bf  88.41 
                                        & 79.67 & \bf  86.12 
                                        & 69.29 & \bf  79.41 \\
                RC2 $\uparrow$          & 96.27 & \bf  97.12 
                                        & 96.17 & \bf  96.98 
                                        & 95.42 & \bf  96.77 
                                        & 91.89 & \bf  95.53 \\
                %\midrule
                \bottomrule
        \end{tabular}
        \caption{Quantitative results at different noise levels of
the input point cloud at each frame.} 
        \label{tab:robust_noise}
        \end{center}
        %\vspace{-8mm}
\end{table}


\begin{table}[!htbp]
	\renewcommand\arraystretch{1.2}
        \setlength{\tabcolsep}{2pt}
	\begin{center}
        \footnotesize
		\begin{tabular}{*{10}{c}}
                \toprule
			\multirow{2}*{Method} & \multicolumn{2}{c}{10,000}   & \multicolumn{2}{c}{5,000}  & \multicolumn{2}{c}{2,500} & \multicolumn{2}{c}{250} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  & NPHM & Ours   & NPHM & Ours   & NPHM & Ours   & NPHM & Ours 	\\
			\midrule
                $\ell_2$ $\downarrow$   & 1.229  & \bf 1.111  
                                        &  1.188 & \bf 1.104  
                                        & 1.226 & \bf 1.108 
                                        & 1.274 & \bf 1.250 \\
                NC $\uparrow$           & 87.79 & \bf 88.71 
                                        & 87.56  & \bf 88.66 
                                        & 87.40 & \bf 88.64 
                                        & 87.22 & \bf 87.80 \\
                RC $\uparrow$           & 84.25 & \bf 89.62 
                                        & 84.49 & \bf 89.87 
                                        & 83.55 & \bf 89.65 
                                        & 81.78 & \bf 85.31 \\
                RC2 $\uparrow$          & 96.16  & \bf 97.15  
                                        & 96.27 & \bf 97.12 
                                        & 96.21 & \bf 97.16 
                                        & 95.74 & \bf 96.22 \\
                %\midrule
                \bottomrule
        \end{tabular}
        \caption{Quantitative results at different sparsity levels of
the input point cloud at each frame.} 
        \label{tab:robust_sparsity}
        \end{center}
\end{table}

==> table/robust_new.tex <==
\begin{table*}[!htbp]
	\renewcommand\arraystretch{1.2}
        \setlength{\tabcolsep}{1.2pt}
        %\setlength{\tabcolsep}{2pt}
	\begin{center}
        \footnotesize
		\begin{tabular}{*{21}{c}}
                \toprule
            \multirow{2}*{Method} & \multicolumn{5}{c}{0}   & \multicolumn{5}{c}{0.5 mm}  & \multicolumn{5}{c}{1mm} & \multicolumn{5}{c}{2mm} \\
    		\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}  
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours 	\\
			\midrule
                $\ell_2$ $\downarrow$   & 1.188  & \bf 1.104 
                                        & 1.231 & \bf 1.146   
                                        & 1.271 & \bf  1.209 
                                        & 1.574 & \bf 1.392 \\
                NC $\uparrow$           & 87.56 & \bf  88.66   
                                        & 87.64 & \bf  88.58 
                                        & 86.89 & \bf  88.50  
                                        & 84.69 & \bf  88.10 \\
                RC $\uparrow$           & 84.49 &  \bf 89.87 
                                        & 82.93 &  \bf  88.41 
                                        & 79.67 & \bf  86.12 
                                        & 69.29 & \bf  79.41 \\
                RC2 $\uparrow$          & 96.27 & \bf  97.12 
                                        & 96.17 & \bf  96.98 
                                        & 95.42 & \bf  96.77 
                                        & 91.89 & \bf  95.53 \\
                %\midrule
                \bottomrule
        \end{tabular}
        \caption{Quantitative results at different noise levels of
the input point cloud at each frame.} 
        \label{tab:robust_noise}
        \end{center}
        %\vspace{-8mm}
\end{table*}


\begin{table*}[!htbp]
	\renewcommand\arraystretch{1.2}
        %\setlength{\tabcolsep}{2pt}
        \setlength{\tabcolsep}{1.2pt}
	\begin{center}
        \footnotesize
		\begin{tabular}{*{21}{c}}
                \toprule
			\multirow{2}*{Method} & \multicolumn{5}{c}{10,000}   & \multicolumn{5}{c}{5,000}  & \multicolumn{5}{c}{2,500} & \multicolumn{5}{c}{250} \\
			\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}  
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours   
                & FLMAE & ImFace* & ImAvatar & NPHM & Ours 	\\
			\midrule
                $\ell_2$ $\downarrow$   & 1.229  & \bf 1.111  
                                        &  1.188 & \bf 1.104  
                                        & 1.226 & \bf 1.108 
                                        & 1.274 & \bf 1.250 \\
                NC $\uparrow$           & 87.79 & \bf 88.71 
                                        & 87.56  & \bf 88.66 
                                        & 87.40 & \bf 88.64 
                                        & 87.22 & \bf 87.80 \\
                RC $\uparrow$           & 84.25 & \bf 89.62 
                                        & 84.49 & \bf 89.87 
                                        & 83.55 & \bf 89.65 
                                        & 81.78 & \bf 85.31 \\
                RC2 $\uparrow$          & 96.16  & \bf 97.15  
                                        & 96.27 & \bf 97.12 
                                        & 96.21 & \bf 97.16 
                                        & 95.74 & \bf 96.22 \\
                %\midrule
                \bottomrule
        \end{tabular}
        \caption{Quantitative results at different sparsity levels of
the input point cloud at each frame.} 
        \label{tab:robust_sparsity}
        \end{center}
\end{table*}
